Leveraging feature communication in federated learning for remote sensing image classification

In the realm of Federated Learning (FL) applied to remote sensing image classification, this study introduces and assesses several innovative communication strategies. Our exploration includes feature-centric communication, pseudo-weight amalgamation, and a combined method utilizing both weights and features. Experiments conducted on two public scene classification datasets unveil the effectiveness of these strategies, showcasing accelerated convergence, heightened privacy, and reduced network information exchange. This research provides valuable insights into the implications of feature-centric communication in FL, offering potential applications tailored for remote sensing scenarios.

==> FigureTables/visfeaturesTex.tex <==
    \begin{tikzpicture} \begin{axis}[%
        enlarge x limits, view={0}{90}, xlabel=$x$, ylabel=$y$, small,
    ]
        \definecolor{color1bg}{HTML}{ECD9ED}
        \addplot3[ contour gnuplot={levels={0.1},labels=false},
                contour/draw color={red!70!black},
                samples=20, samples y=20, %
            ]{e^(-(  1*(x-1)^2  +   2*0*(x-1)*(y-3)   +   2*(y-3)^2    ))};
        \addplot3[ contour gnuplot={levels={0.1},labels=false},
                contour/draw color={blue!70!black},
                samples=20, samples y=20, %
            ]{e^(-(  2*(x-3)^2  +   2*0*(x-3)*(y-4)   +   3*(y-4)^2    ))};
        \addplot+[only marks, scatter, mark size=2pt,
            scatter/classes={A={mark=+,red!70!black},
                           cntA={mark=oplus,red!70!black, thick},
                             B={mark=+,blue!70!black},
                           cntB={mark=oplus,blue!70!black, thick},
                           Cnt={mark=oplus,green!50!black, thick, mark size=3pt}
            },
            scatter src=explicit symbolic
        ]table[x index=0, y index=1, meta index=2] {
                x       y       label
                1       3       cntA
                1.5     3.5     A
                0.5     2.5     A
               -0.3     3.0     A
                2.3     3.0     A
                3       4       cntB
                3.2     4.2     B
                2.8     3.8     B
                3.5     3.7     B
                2.5     4.2     B
                2       3.5     Cnt
            };
        \addplot3[ contour gnuplot={levels={0.1},labels=false},
                contour/draw color={red!70!black},
                samples=20, samples y=20,
            ]{e^(-(  2*(x-0)^2  +   2*0*(x-0)*(y-0)   +   4*(y-0)^2    ))};
        \addplot3[ contour gnuplot={levels={0.1},labels=false},
                contour/draw color={blue!70!black},
                samples=20, samples y=20,
            ]{e^(-(  1*(x-2)^2  +   2*0*(x-2)*(y+1)   +   3*(y+1)^2    ))};
        \addplot+[only marks, scatter, mark=x, mark size=2pt,
            scatter/classes={A={mark=x,red!70!black},
                           cntA={mark=otimes,red!70!black, thick},
                             B={mark=x,blue!70!black},
                           cntB={mark=otimes,blue!70!black, thick},
                           Cnt={mark=otimes,green!50!black, thick, mark size=3pt}
            },
            scatter src=explicit symbolic
        ]table[x index=0, y index=1, meta index=2] {
                x       y       label
                0.3     0.1     A
               -0.3    -0.1     A
                1.5    -1.3     B
                2.5    -0.7     B
                0       0       cntA
                2      -1       cntB
                1      -0.5     Cnt
            };
        \end{axis}
    \end{tikzpicture}

